Structured Depth Prediction in Challenging Monocular Video Sequences

In this paper, we tackle the problem of estimating the depth of a scene from a monocular video sequence. In particular, we handle challenging scenarios, such as non-translational camera motion and dynamic scenes, where traditional structure from motion and motion stereo methods do not apply. To this end, we first study the problem of depth estimation from a single image. In this context, we exploit the availability of a pool of images for which the depth is known, and formulate monocular depth estimation as a discrete-continuous optimization problem, where the continuous variables encode the depth of the superpixels in the input image, and the discrete ones represent relationships between neighboring superpixels. The solution to this discrete-continuous optimization problem is obtained by performing inference in a graphical model using particle belief propagation. To handle video sequences, we then extend our single image model to a two-frame one that naturally encodes short-range temporal consistency and inherently handles dynamic objects. Based on the prediction of this model, we then introduce a fully-connected pairwise CRF that accounts for longer range spatio-temporal interactions throughout a video. We demonstrate the effectiveness of our model in both the indoor and outdoor scenarios.

==> abstract14.tex <==
\begin{abstract}

In this paper, we tackle the problem of estimating the depth of a scene from a single image. This is a challenging task, since a single image on its own does not provide any depth cue. To address this, we exploit the availability of a pool of images for which the depth is known. More specifically, we formulate monocular depth estimation as a discrete-continuous optimization problem, where the continuous variables encode the depth of the superpixels in the input image, and the discrete ones represent relationships between neighboring superpixels. The solution to this discrete-continuous optimization problem is then obtained by performing inference in a graphical model using particle belief propagation. The unary potentials in this graphical model are computed by making use of the images with known depth. We demonstrate the effectiveness of our model in both the indoor and outdoor scenarios. Our experimental evaluation shows that our depth estimates are more accurate than existing methods on standard datasets.

\end{abstract}


==> abstract15.tex <==
\begin{abstract}
\label{sec:abstract}

In this paper, we tackle the problem of estimating the depth maps of the frames of a monocular video sequence. In particular, we focus on the scenarios where traditional structure-from-motion and motion stereo fail, such as in the presence of moving objects and videos captured by a non-translational camera. To this end, we introduce a structured prediction approach that allows us to reason about local geometry and motion, while modeling complex spatio-temporal relationships between neighboring regions within an image and across images. In particular, we design a two-frame model that naturally encodes short-range temporal consistency and inherently handles dynamic objects. Based on the prediction of this model, we then introduce a fully-connected pairwise CRF that accounts for long-range spatio-temporal interactions throughout a video. We demonstrate the benefits of our approach on the MSR-V3D dataset, where we achieve state-of-the-art accuracy.

%In this paper, we introduce a method to estimate the depth maps of the frames in a video sequence. In particular, we tackle the scenarios where traditional structure-from-motion and motion stereo methods fail, such as in the presence of dynamic  videos and videos captured by a non-translational camera. To address this challenging problem, we adopt a non-parametric approach, which utilizes a pool of video sequences with known depths.  We first design a two-frame model which exploits the information contained in every two consecutive images and lets us naturally encode temporal consistency. In this setting, we further introduce a motion-aware energy function that allows us to effectively handle dynamic foreground objects. Given the estimated depth for each frame, we finally apply a post-processing procedure which utilizes a fully connect CRF model with Gaussian edge potentials to enforce long range temporal consistency. We demonstrate the effectiveness of our approach on the MSR-V3D dataset and show that our model achieves state-of-the-art accuracy.
\end{abstract}

==> deriveg.tex <==
\section{Gradient for Projected Hellinger Distance} %\ref{}}
\label{deriveg}
In subspace learning approach, the gradient of the objective function with respect to $\Mat{W}$ is in the form of:
\begin{equation*}
\frac{\partial \hat{D}}{\partial \Mat{W}}= \frac{1}{n_s}\sum_{i=1}^{n_s}\frac{\partial \hat{G}}{\partial \hat{T}}\frac{\partial \hat{T}}{\partial \Mat{W}}\mid x_i^s + \frac{1}{n_t}\sum_{i=1}^{n_t}\frac{\partial \hat{G}}{\partial \hat{T}}\frac{\partial \hat{T}}{\partial \Mat{W}}\mid x_i^t
\end{equation*}
%with $G=(\sqrt{\hat{T}(x_i^f)}-\sqrt{1-\hat{T}(x_i^f)}$
in which $\frac{\partial T}{\partial \Mat{W}}$ can be estimated as:
\begin{equation*}
\frac{\partial T}{\partial \Mat{W}} = T(1-T)(\frac{\partial \log \hat{s}}{\partial \Mat{W}}-\frac{\partial \log \hat{t}}{\partial \Mat{W}})
\end{equation*}
It can be shown that
\begin{equation*}
\hat{T}(1-\hat{T})\frac{\partial \hat{G}}{\partial \hat{T}}=\sqrt{\hat{T}(1-\hat{T})}(2\hat{T}-1)
\end{equation*}
which thus yields:%, our gradient can be re-written as:
\begin{eqnarray}
     \frac{\partial \hat{D}}{\partial \Mat{W}}\hspace{-0.3cm} &= &\frac{1}{n_s}\sum_{i=1}^{n_s}\sqrt{\hat{T}(1-\hat{T})}(2\hat{T}-1)(\frac{\partial \log \hat{s}}{\partial \Mat{W}}-\frac{\partial \log \hat{t}}{\partial \Mat{W}})\mid x_i^s \nonumber\\
    &+&\hspace{-0.3cm}\frac{1}{n_t}\sum_{i=1}^{n_t}\sqrt{\hat{T}(1-\hat{T})}(2\hat{T}-1)(\frac{\partial \log \hat{s}}{\partial \Mat{W}}-\frac{\partial \log \hat{t}}{\partial \Mat{W}})\mid x_i^t \nonumber \;,
    \label{eqn:SSA_KL2}
\end{eqnarray}
%which requires computing the gradient of $\frac{\partial \log \hat{s}(\Mat{W}^T x)}{\partial \Mat{W}} \mid x^s$ and $\frac{\partial \log \hat{t}(\Mat{W}^T x)}{\partial \Mat{W}} \mid x^t$. This gradient for $\frac{\partial \log \hat{s}(\Mat{W}^T x)}{\partial \Mat{W}}$ can be computed as:
which requires computing four intermediate gradients of the form $\frac{\partial \log \hat{f}(\Mat{W}^T x)}{\partial \Mat{W}} \mid x^f$ where $f$ is either $s$ or $t$. Here, we show how to derive the first gradient, and following this all the remaining three gradients can be computed:
\begin{small}
\begin{eqnarray}
    \frac{\partial \log \hat{s}(\Mat{W}^T x)}{\partial \Mat{W}}\mid x^s \hspace{-0.3cm} &= & \hspace{-0.3cm} \frac{\partial}{\partial \Mat{W}} \log \left( \frac{1}{n_s} \sum_{i=1}^{n_s} \frac{1}{\sqrt{2\pi \Mat{H}_{\Mat{W}}}} k(x,x_i^s) \right ) \nonumber \\
    \hspace{-0.3cm} &= &\sum_{i=1}^{n_s} -\bar{A}_i^s  (x-x_i^s) (x-x_i^s)^T \Mat{W} \Mat{H}_{\Mat{W}}^{-1}\nonumber \\
    \hspace{-0.3cm} &= & - \Mat{C}^s(x) \Mat{W} \Mat{H}_{\Mat{W}}^{-1}  \;,
    \label{eqn:SSA_KL2}
\end{eqnarray}
\end{small}
Here, we can define: %$k$ is the Guassian kernel of projected samples:
\begin{flalign*}
\hspace{-0.5cm} k(x,x_i^s)=\exp \left( \frac{-(x-x_i^s)^T \Mat{W} \Mat{H}_{\Mat{W}}^{-1} \Mat{W}^T(x-x_i^s)}{2}  \right ) \;
\end{flalign*}
\vspace{-0.3cm}
\begin{flalign*}
\hspace{-0.5cm} \bar{A}_i^s=\frac{k(x,x_i^s)}{\sum_{i=1}^{n_s} k(x,x_i^s)} \hspace{0.1cm};\hspace{0.1cm}\hspace{0.1cm} \Mat{C}^s(x)=\sum_{i=1}^{n_s} \bar{A}_i^s (x-x_i^s) (x-x_i^s)^T \;
\end{flalign*}
and $\Mat{H}_\Mat{W}$, the diagonal matrix whose elements derived from projected source and target samples with MSP algorithm.
% \mbox{{$k(\Mat{W}^T x,\Mat{W}^T x_i^s)=\exp \left( \frac{-(x-x_i^s)^T \Mat{W} \Mat{H}_{\Mat{W}}^{-1} \Mat{W}^T(x-x_i^s)}{2}  \right )$}},  \mbox{$\bar{A}_i^s=\frac{k(\Mat{W}^T x,\Mat{W}^T x_i^s)}{\sum_{i=1}^{n_s} k(\Mat{W}^T x,\Mat{W}^T x_i^s)}$}, \mbox{$\Mat{C}^s(x)=\sum_{i=1}^{n_s} \bar{A}_i^s (x-x_i^s) (x-x_i^s)^T$} and $\Mat{H}_\Mat{W}$ is the diagonal matrix with diagonal elements derived from projected source and target samples with MSP algorithm. our final Gradient will take the form of:
%\begin{equation*}
%\bar{A}_i^f=\frac{\exp\left(\frac{-(x-x_i^f)^T \Mat{W} H_f^{-1} \Mat{W}^T(x-x_i^f)}{2} \right )}{\sum_{j=1}^{n_f} \exp\left(\frac{-(x-x_j^f)^T \Mat{W} H_f^{-1} \Mat{W}^T(x-x_j^f)}{2} \right )}
%\end{equation*}
%Finally Gradient of $\frac{\partial \hat{D}}{\partial W}$ will take the form of:
Our final Gradient will take the form of:
\begin{small}
\begin{eqnarray}%\Mat{H}_\Mat{W}\frac{\partial \Mat{H}_\Mat{W}}{\partial W}
\hspace{-0.1cm}\frac{\partial \hat{D}}{\partial \Mat{W}} &=&\hspace{-0.1cm}\frac{1}{n_s}\sum_{i=1}^{n_s}\sqrt{\hat{T}(x_i^s)(1-\hat{T}(x_i^s))}(2\hat{T}(x_i^s)-1) \nonumber\\
\hspace{-0.1cm} & \times &\hspace{-0.1cm} \left[(-\Mat{C}^s(x_i^s) + \Mat{C}^t(x_i^s)) \Mat{W}\Mat{H}_\Mat{W}^{-1} \right. \nonumber\\
\hspace{-0.1cm} & + & \left. \hspace{-0.1cm} \frac{\partial \Mat{H}_\Mat{W}^{-1}}{\partial \Mat{W}}(-A^s(x_i^s) k(x^s_i,*) +  A^t(x_i^s)k(x^s_i,*))\right] \nonumber\\
\hspace{-0.1cm} &+&\hspace{-0.1cm}\frac{1}{n_t}\sum_{i=1}^{n_t}\sqrt{\hat{T}(x_i^t)(1-\hat{T}(x_i^t))}(2\hat{T}(x_i^t)-1) \nonumber \\
\hspace{-0.1cm} & \times &\hspace{-0.1cm} \left[(-\Mat{C}^s(x_i^t) + \Mat{C}^t(x_i^t)) \Mat{W}\Mat{H}_\Mat{W}^{-1} \right.  \nonumber \\
\hspace{-0.1cm} & + &\hspace{-0.1cm} \left. \frac{\partial \Mat{H}_\Mat{W}^{-1}}{\partial \Mat{W}}(-A^s(x_i^t) k(x^s_i,*) +  A^t(x_i^t)k(x^t_i,*))\right] \nonumber \;
\end{eqnarray}
\end{small}

%\begin{equation*}
%\bar{A}_i^s=\frac{\exp\left(\frac{-(x-x_i^s)^T \Mat{W} H^{-1} \Mat{W}^T(x-x_i^s)}{2} \right )}{\sum_{j=1}^{n_s} \exp\left(\frac{-(x-x_j^s)^T \Mat{W} H^{-1} \Mat{W}^T(x-x_j^s)}{2} \right )}
%\end{equation*} and $\bar{A}_i^s=\frac{\Mat{K}(x^s_i,*)}{\sum_{j=1}^{n_s}\Mat{K}(x^s_i,*)}$.



